A Review on Language Models as Knowledge Bases

Recently, there has been a surge of interest in the NLP community on the use of pretrained Language Models (LMs) as Knowledge Bases (KBs). Researchers have shown that LMs trained on a sufficiently large (web) corpus will encode a significant amount of knowledge implicitly in its parameters. The resulting LM can be probed for different kinds of knowledge and thus acting as a KB. This has a major advantage over traditional KBs in that this method requires no human supervision. In this paper, we present a set of aspects that we deem a LM should have to fully act as a KB, and review the recent literature with respect to those aspects.

==> 8_models.tex <==
\section{Models}
\input{tables/models}


In the previous sections, we detail more general aspects of LMs. In this section, we cover the different models that fall under the \lmkb paradigm and the solutions proposed by these models that improve LM performance.

These models often incorporate knowledge explicitly through several means: via some form of \textbf{pretraining} strategy that explicitly encodes entity-level or relation-level data or via the integration of \textbf{external memory} to an existing LM. Models that implicitly contain knowledge, such as existing pretrained LMs, are not covered in this section, as we focus on explicit incorporation of knowledge.



% - external memory
% --> via external knowledge graphs
% --> via parametric memory
% --> via additional attention mechanisms?

% - pretraining
% --> pretraining on entities
% --> pretraining on relations
% --> pretraining on ???

\subsection{External Memory} Existing LMs are often unable to store localized information about facts and specific knowledge; on the other hand, KBs have been known to store information about millions of entities. Knowing this, existing research has focused on taking advantage of the storage capabilities of existing KBs and integrating this capability into LMs \cite{wei2021knowledge}.

\citet{heinzerling_language_2021} introduced initial work understanding how \lmkb can be used in more general settings, especially in integrating knowledge about general and rare entities, since representing millions of entities within LMs is difficult when LMs have a limited vocabulary. Current work often forgoes the potential to deploy these \lmkb in the real world. To improve existing LM and overcome memory limitations, current work has focused on the goal of improving memory for LMs to store more information about external information, such as information about entities in a sentence.

External memory has previously been used for neural networks \cite{Bahdanau2015NeuralMT, weston2015memory, graves2014neural, ahn2017neural}. \citet{ahn2017neural} specifically proposed the \newterm{Neural Knowledge Language Model} (NKLM) to take advantage of external knowledge and exploit factual knowledge. Since then, a large number of works have focused on the integration of this external memory to improve performance on knowledge-intensive tasks. To summarize these works, we focus on detailing the different strategies of integrating external memory within LMs and how they can be further improved on.

\subsubsection{External Knowledge Graphs}
Much work prior to the focus on \lmkb focus on the integration of KBs explicitly within LMs. Thus, Knowledge Enhanced Pretrained LMs \newterm{KE-PLM} \cite{wei2021knowledge} have become the backbone of models that integrate knowledge explicitly. 

External knowledge graphs (KGs) have been known to 

\subsubsection{Parametric, Semiparametric, and Non-Parametric Memory}
We focus on parametric, semi-parametric, and non-parametric memories integrated within LMs. \textbf{Parametric memory} can be seen as memory latent within LMs; \textbf{non-parametric memory} can be seen as memory that is used in addition to internal LM memory; and \textbf{semiparametric memory} can be seen as a combination of both parametric memory and non-parametric memory.

\paragraph{Parametric Memory}

\paragraph{Non-Parametric Memory}

\paragraph{Semiparametric Memory} \citet{yogatama_adaptive_2021} introduce the idea of semiparametric memory.

\subsubsection{Attention over Memory}


\subsection{Pretraining}
Models have been known to encode knowledge within their parameters through unsupervised methods, specifically pretraining. For example, given the example \texttt{Obama is from [MASK]}, using a masked language modeling (MLM) objective, we would expect the model to predict \texttt{Hawaii}. However, there is no explicit integration of any entity-level or relation-level knowledge through this objective. As a result, a number of works have sought to incorporate entity-level or relation-level knowledge through pretraining strategies and loss function modifications. 

==> 8_tasks.tex <==
\section{Tasks}
As a starting point, we detail the different tasks and models that have been designed to get closer to the goal of \lmkb. One challenge of this is the fact that there does not currently exist standardized benchmarks for \lmkb, likely owing to the fact that knowledge latent within LMs can be measured in a multitude of tasks. However, our goal is to delineate a set of tasks that can be used initially as measurements to achieve this goal.



==> Survey_ LMs as KB/1_introduction.tex <==
\section{Introduction}

% The impact pre-trained Language Models (\newterm{LMs}) have had on Natural Language Processing (\newterm{NLP}) can be described as nothing short of transformative. It has dramatically changed the way we do NLP research. The field moved from \textit{feature} \cite{och-etal-2004-smorgasbord, zhang-nivre-2011-transition} and \textit{architecture engineering} \cite{Chung2014EmpiricalEO, kim-2014-convolutional, Bahdanau2015NeuralMT, vaswani17attention} to the \textit{pre-train and fine-tune} paradigm \cite{Radford2018ImprovingLU, dong_NEURIPS2019_c20bb2d9, lewis_retrieval-augmented_2021}, and lately to the \textit{pre-train, prompt and predict} paradigm, aka ``in-context" learning \cite{Liu2021PretrainPA}. Recently, LMs have been disrupting another technology that has been stale for years and that is of Knowledge Bases (\newterm{KBs}). In a seminal work, \citet{petroni_language_2019} show that LMs not only store vast amounts of linguistic knowledge in its parameters \cite{} but also relational knowledge; thus having the potential to serve as KBs.  


The impact of Pretrained Language Models (\newterm{LMs}) on Natural Language Processing (\newterm{NLP}) research can be described as nothing short of transformative. It has moved the field from \textit{feature engineering}  \cite{och-etal-2004-smorgasbord, zhang-nivre-2011-transition} and \textit{architecture engineering} \cite{Chung2014EmpiricalEO, kim-2014-convolutional, Bahdanau2015NeuralMT, vaswani17attention} to the \textit{pre-train and fine-tune} paradigm \cite{Radford2018ImprovingLU, dong_NEURIPS2019_c20bb2d9, lewis_retrieval-augmented_2021}, and lately the \textit{pre-train, prompt, and predict} paradigm \cite{Liu2021PretrainPA}. LMs pretrained on a large corpus of web data have been shown to contain different kinds of knowledge implicitly in their parameters without the need for any human supervision. This includes: world knowledge \cite{petroni_language_2019, rogers_primer_2020}, relational knowledge \cite{safavi2021relational}, commonsense knowledge \cite{Da2021AnalyzingCE}, linguistic knowledge \cite{Peters2018DissectingCW, Goldberg2019AssessingBS, tenney2018what}, actionable knowledge \cite{Huang2022LanguageMA} and more. This access to knowledge is crucial for LMs to achieve state-of-the-art results on various downstream tasks. However, as is the case with most neural systems, knowledge in LMs is encoded in a diffused manner, making it generally difficult to interpret and hard to update.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/lm-as-kbs-1.pdf}
    \caption{Aspects of \lmkb as presented in this work}
    \label{fig:lmkb}
\end{figure}

Despite these recent breakthroughs, we often do not have full control over the behavior of LMs. As a result, utilizing these models in real-world scenarios is often unsuccessful. On the other hand, Knowledge Bases (\newterm{KB}) are easier to control. Here, KBs refers to a data structure that stores relational information in the form of triples connecting two triplets of entities by symbolic relations (e.g. $\langle$ \texttt{Cairo}, \texttt{CapitalOf}, \texttt{Egypt} $\rangle$). They often follow rule-based heuristics, rendering them predictable, in addition to possessing large knowledge coverage, which primes them for use in real-world systems. These models are often used as chatbots and virtual assistants, where controlled generation of output is necessary to ensure appropriate responses \cite{chen-dialogue-2017}. Therefore, KBs are a natural solution to access specific gold-standard relational information. They are repositories of knowledge, for both structured and unstructured data, and can be seamlessly queried and updated by an end user. 

% KBs have traditionally been used in artificial intelligence research in the context of expert systems since they provide an effective way to add, remove, or replace annotated relational data as the location of the knowledge is readily apparent. 

Since KBs can access and update relational knowledge easier than LMs can, one question naturally arises: how can we control the repository of knowledge stored implicitly in the weights of a LM as similarly as KBs can? This question was first introduced in seminal work by \citet{petroni_language_2019} and has since ignited the interest of the community with the goal of instilling LMs with desirable properties of KBs.

Several works have already approached improving LMs through the lens of KBs: \citet{petroni_language_2019, dhingra_time-aware_2021, wang_language_2020, heinzerling_language_2021, sung2021language}. Many of these works include updating factoids stored within the parameters of LMs \cite{de_cao_editing_2021, mitchell_fast_2021, hase_language_2021} to creating new methods for extracting factual knowledge \cite{petroni_language_2019}. Despite significant progress towards achieving parity between LMs and KBs, LMs still lack specific aspects that KBs have. For example, given the cloze phrases ``\texttt{Albert Einstein was born in [MASK]}'' and ``\texttt{The hometown of Albert Einstein is [MASK]}'', a user of a KB can map both queries to one triplet $\langle$ \texttt{Albert Einstein}, \texttt{BornIn}, \textbf{X} $\rangle$ that the KB readily understands and thus consistently returns the same city. On the other hand, LMs may not be as consistent, yielding potentially different answers for the same underlying factual questions. 

In this survey, we propose to consolidate the work on \texttt{LMs-as-KBs} within one cohesive framework, with a focus on aspects related to KBs that we think are useful to integrate into LMs. Few survey papers exist that evaluate LMs in this context. For instance, \citet{wei2021knowledge} evaluate knowledge-enhanced pretrained LMs by delineating the types of knowledge that can be integrated into existing LMs. \citet{safavi2021relational} divide relevant work according to the level of supervision provided to the LM by a KB. Similarly, \citet{colonhernandez2021combining} cover the integration of structural knowledge into LMs but forgo implicit knowledge. Our study of \lmkb from our perspective is unique compared to the focus of existing survey papers. We aim to present the current landscape of \lmkb research and highlight the existing challenges that LMs face when applied in practice. 

% By following these goals, we bring years of research on KBs together for improving usability of LMs in practice.

We observe the recent advances in LMs and explore them with respect to aspects that we find necessary for LMs to become as functional and utilizeable as KBs: \textit{access}, \textit{consistency}, \textit{editability}, \textit{reasoning}, and \textit{explainability}. We further highlight where we are now in terms of the \lmkb framework as well as potential work for the future. Finally, we discuss the remaining challenges in the full adoption of \lmkb and propose directions for future research. This survey is structured as follows:

\begin{enumerate}
    \item First, an overview of KBs and LMs and their intersection for \lmkb
    \item Second, the enumeration of the aspects of \lmkb
    \item Third, a brief summarization of each aspect with respect to recent work
    % \item Third, a brief summarization of each aspect in conjunction with work necessary to improve the aspect
    % \item Fourth, explanations of the potential for future work
\end{enumerate}

% In short, our contributions in this paper are as follows:

% \begin{enumerate}
%     % \item We survey \lmkb from the viewpoint of knowledge latent in the LMs, rather than from knowledge explicitly given to LMs.
%     \item We identify aspects to categorize existing LMs ??
%     \item We compile a list of papers for each aspect of LMs we find useful in understanding the landscape of the field of research
    
%     % \item We create a paradigm in which to divide up current LMs 
%     % \item We enumerate the aspects of KBs that are currently lacking in LMs and suggest ways to improve current work.
%     % \item We provide recommendations towards a standard set of benchmarks and tasks that are ideal to establishing \lmkb.
%     % \item We provide a list of current models that work towards the goal of building \lmkb.
% \end{enumerate}

% We hope that by highlighting the framework for \lmkb, we can consolidate knowledge in this ever-growing field of research and further emphasize the necessity of improving on these aspects within LMs for future real-world applications. 

We hope that by highlighting the aspects of \lmkb, we can consolidate knowledge in this ever-growing field of research. We envision that our work can provide a path for those new to the area of research to better improve LMs to be just as good, if not eventually better, than KBs.

% Furthermore, our goal is to introduce a path forward for beginners interested in understanding how to better improve LMs to be just as good, but eventually better, than KBs. 





%%%%%%%%% TO ADD IN BACKGROUND %%%%%%%%%  
% Existing work has focused on the integration of KBs into current LMs for paradigms such as reinforcement learning \cite{bahdanau2019learning, branavan-etal-2011-learning, chevalierboisvert2019babyai, luketina2019survey}, commonsense reasoning \cite{ji2020language, zellers2019recognition, talmor-etal-2019-commonsenseqa}, representation learning \cite{shen2020exploiting} and more. 

%%%%%%%%% Archive %%%%%%%%%  
% We approach LMs through the lens of KBs, showing how similar functionality in LMs is to the functionality of KBs and the attributes in KBs that are necessary to adopt in LMs to improve the \lmkb framework

==> Survey_ LMs as KB/2_preliminaries.tex <==
\section{Preliminaries}
In this section, we define what LMs and KBs are, characterize the functions and attributes of KBs, and make direct comparisons between both LMs and KBs to highlight the current limitations of LMs in the context of the \lmkb framework.

\subsection{Knowledge Bases}
\label{sec:kbs}
% The term KB refers to a data structure that stores relational information in the form of triples connecting pairs of entities by symbolic relations (e.g. $\langle$ \texttt{Cairo}, \texttt{CapitalOf}, \texttt{Egypt} $\rangle$). 
KBs usually adhere to a manually engineered schema that dictates the possible set of entities and relations and the interactions between them. Such a rigid schema facilitates different kinds of complex operations over the data (e.g. multi-hop reasoning) and ensures accurate, consistent and explainable answers. Examples of KBs include Wikidata \cite{wikidata} and the ATOMIC \cite{sap2019atomic} (See Appendix \ref{app:kgs} for further details).    

% A KB naturally has the ability to \textbf{query} for fill-in-the-blanks answers. For example, given (\texttt{Albert Einstein}, \texttt{born-in}, \textbf{X}), we have a relation triplet of the form \textit{(h, r, t)} with a head entity \textit{h}, relation \textit{r}, and entity \textit{t}, and the KB can predict the corresponding tail entity \textit{t}.

% Given the same example above, we can \textbf{update} either the entities or relations such that we choose a new one and make a prediction based off the swapped entity. For example, instead of (\texttt{Albert Einstein}, \texttt{born-in}, \textbf{X}), we would have (\texttt{Isaac Newton}, \texttt{born-in}, \textbf{X}), and the KB would be able to make the correct prediction of \textbf{England}.

% However, current LMs are limited in \textbf{querying} responses for cloze statements since the prediction may be spurious or out of context. For example, given the previou relation triplet (\texttt{Albert Einstein}, \texttt{born-in}, \textbf{X}) written in full as a cloze statement \texttt{“Albert Einstein was born in [MASK]”}, existing LMs may be unable to complete the blank with a word such as "Germany" and instead choose a word such as "nearby," which is thoroughly out of context and factually incorrect.

% Furthermore, \textbf{updating} the existing knowledge in the parameters of LMs is not as simple as finding the location of the relation triplet, as it would be for KBs. Because LMs in the present day have billions of parameters (or more) that store knowledge in an opaque manner, current vanilla LMs are unable to satisfy the ability to update outdated knowledge.

\subsection{Language Models}
In the context of this paper, we use the term ``LM" to refer to a deep neural LM that is pre-trained on a large amount of unlabeled text in a self-supervised setting such as masked language modeling. Examples include transformer-based models \cite{vaswani17attention} such as BERT \cite{devlin-etal-2019-bert}, GPT-3 \cite{gpt3}, BART \cite{lewis-etal-2020-bart} and T5 \cite{Raffel2020ExploringTL}. 


% Note that we only consider LMs as a standalone system without access to any explicit knowledge sources, as compared to existing work that has focused on augmenting LMs with external KBs to improve their capabilities on downstream tasks.

\subsection{LMs-as-KBs}
% We also define KBs in terms of the \textbf{attributes} that are inherent in existing KBs. 
% TALK ABOUT A REAL KNOWLEDGE BASE W/ RESPECT TO THE ATTRIBUTES LISTED
% However, KBs lacks the flexibility that LMs offer in terms of extendability and expressability. KBs also require significant human effort to build and maintain. For example, populating KBs involves extracting huge amounts of relational data from unstructured text by using complex NLP pipelines such as entity linking and coreference resolution \cite{petroni_language_2019}. In contrast, LMs are able to implicitly capture this information without any supervision.

KBs lack the flexibility that LMs offer in terms of extendability and expressability. KBs also require significant human effort to build and maintain. For example, populating KBs involves extracting huge amounts of relational data from unstructured text by using complex NLP pipelines such as entity linking and coreference resolution \cite{petroni_language_2019}. In contrast, LMs are able to implicitly capture this information without any supervision. 

To better frame the current limitations of LMs with respect to the capabilities of KBs, we observe a total of five aspects of KBs that we would like LMs to excel at in order to be considered a KB. We consider \textbf{Access}, \textbf{Edit}, \textbf{Consistency}, \textbf{Reasoning}, and \textbf{Explainability and Interpretability}. The latter three are not implicitly done, but are easier to ensure within KBs than LMs.

% In particular, \textbf{Access} and \textbf{Edit} are two aspects that are implicit in KBs that LMs can improve on. Furthermore, we denote three more aspects that we find are easier to ensure within KBs than in LMs, though are not automatically implicitly done: \textbf{Consistency}, \textbf{Reasoning}, and \textbf{Explainability}. We highlight these aspects to promote framing the question from a KBs standpoint to overall LMs.

% To better frame the current limitations of LMs with respect to the capabilities of KBs, we define the following features of KBs that we would like LMs to be excelling at in order to be considered as a KB.

% \paragraph{Storage}
% % Define control?
% It is often more difficult to extract and store knowledge in LMs because we often have less control over the knowledge stored within the parameters, and this knowledge is often not localized to specific regions. It tends to be easier in KBs because the location of the knowledge is readily available and that localization is unnecessary as the information is easily readable.

\paragraph{Access}
KBs are often simple to access via manual querying of terms using specific querying languages. On the other hand, LMs cannot be queried explicitly as the knowledge is not directly encoded in specific locations in the model. Current research has focused on \textit{how} we can query LMs similarly to how we can query KBs, focusing on specific access patterns for different types of knowledge. For example, knowledge encoded in LMs can be accessed through probing via fill-in-the-blank (cloze) prompts \cite{taylor1953cloze} and through traditional downstream finetuning. However, there is still more work needed to improve LMs for efficient and direct access.

% directly query for wanted knowledge, as LMs contain a large amount of knowledge latent within their parameters that can be accessed via downstream tasks. However,     it is often difficult to pinpoint the location of where the specific knowledge can be accessed. 

% Knowledge encoded in LMs can be accessed in a multitude of ways, including probing via fill-in-the-blank (cloze) prompts \cite{taylor1953cloze}, by question answering \cite{richardson-sabharwal-2020-qa}, language modeling \cite{Bengio03}, and more, rendering  them more expressive than KBs. However, even though KBs can only be queried through standardized methods, they naturally encode relationships between entities, making them easier to pinpoint and trace back entity-related knowledge. 

% However, despite the ability to access LMs in different ways, they are often limited in the storage capacities that KBs naturally hold \cite{heinzerling_language_2021}. In addition, a key motivation for improving LM access to knowledge is to harness expressivity in a LM and to retain the storage capacity of a KB.

% - Kbs naturally encode entity and relations
% - LMs are more mysterious in how they encode relationships
% - The strength of a KB is its ability to access directly entities and their relationships
% - It's more difficult to do so with an LM because of 1) less storage capacity for direct relationships with entities and relations, and 2) interpretability issues (see explainability)
% - Therefore, it's important to be able to improve LMs in such a way that improves access to specific entity-level knowledge and at the same time keep the expressivity latent in LMs


\paragraph{Edit}
Since LMs are pre-trained on a certain snapshot of data from a specific time, the knowledge it learns can be outdated (e.g. the population of some country), incorrect \cite{Lin2021TruthfulQAMH}, biased or toxic \cite{Gehman2020RealToxicityPromptsEN, bender21}. Perhaps more importantly, in the context of privacy, LMs may memorize sensitive information that needs to be removed \cite{carlini_extracting_2021}. Further, new information is created all the time. For example, most available LMs today would have never seen information related to the COVID-19 Omicron variant. However, updating a specific fact in a LM is not straightforward, as facts are encoded in the weights of the model in a distributed fashion, making them inaccessible or uninterpretable \cite{mitchell_fast_2021}. The naive way of re-training the whole model on an updated set is expensive, especially with the ever-increasing size of current LMs \cite{gpt3}. There are increasing evidence that show that scaling LMs to larger sizes is not the solution to generating factually correct information \cite{lazaridou_mind_2021, Gehman2020RealToxicityPromptsEN, Lin2021TruthfulQAMH}. As a result, this would also result in catastrophic forgetting \cite{wallat_bertnesia_2021}. Changing a single weight may have a ripple effect that affects a large number of other implicitly memorized facts. Therefore, this task of knowledge editing is of utmost importance, especially when considering LMs in the context of KBs.

\paragraph{Consistency}
Language is multifaceted: the same meaning can be expressed in multiple forms. Structured KBs are built with consistency in mind; several efficient algorithms have been proposed to detect inconsistencies in KBs \cite{andersen01} so such conflicts can be easily resolved, while other work aimed at quantifying the degree of which inconsistency arises in KBs \cite{muino11}. Therefore, in the face of such language variability, we should expect LMs to behave consistently under semantically equivalent contexts, even across different languages. Note that consistency does not imply correctness, as a KB can be consistent but store factually incorrect information. Similarly, a LM can have an incorrect belief about a certain fact but that belief is consistent across different queries. 

\paragraph{Reasoning}

% \cite{west_symbolic_2021, talmor_leap--thought_2020, talmor_olmpics_2020, hase_language_2021}
In a KB, it can be simple to follow the path of reasoning. For instance, given the KB triplet $\langle$ \texttt{Cairo}, \texttt{CapitalOf}, \texttt{Egypt} $\rangle$, the KB can sensibly reason that \texttt{Cairo} is in \texttt{Africa} given that it has another relation explicitly stating that \texttt{Egypt} is a part of \texttt{Africa}. On the other hand, recent work has shown that LMs can perform different forms of reasoning when finetuned on datasets that elicit reasoning capabilities within LMs \cite{west_symbolic_2021, talmor_leap--thought_2020, talmor_olmpics_2020, hase_language_2021}. Reasoning is not readily obvious and difficult to facilitate, as LMs have been shown to perform poorly on some types of reasoning such as structured reasoning \cite{kassner2020negated}.

\paragraph{Explainability and Interpretability}
Given a KB triplet, nodes and links can easily be identified, and the answer can easily be inferred. However, in LMs, knowledge is rarely understood by simply looking at the output. Moreover, the location of the parameters in which the knowledge comes from is unknown. Under perfect circumstances, one would want LMs to be explainable and interpretable to the end user, especially for stakeholders with no prior understanding of NLP \cite{Lakkaraju2022RethinkingEA}. However, current research on LMs is far from achieving this goal, as many of the newer techniques focus on black box rather than white box techniques \cite{danilevsky_survey_2020}. As a result, imbuing explainability and interpretability in LMs is core to improve \lmkb. We make the distinction, however, that KBs are inherently explainable. On the other hand, interpretability, while not latent in KBs, is still an important aspect to apply to LMs \cite{Lipton2018TheMO} that we also focus on for the purposes of the survey.



% \paragraph{Consistency}
% Consistency in KBs is important in the sense that given two similar cloze statements, KBs are able to map the statements to a single KB triplet. Given the same example from above for (\texttt{Albert Einstein}, \texttt{born-in}, \textbf{X}), a KB will always return the same answer for \textbf{X}.

% Language is complex, and the same meaning can be expressed in multiple different forms. Therefore, in the face of such language variability, we should expect LMs to behave consistently under semantically equivalent contexts. On the other hand, structured KBs are built with consistency in mind; several efficient algorithms have been proposed to detect inconsistencies in KBs \cite{andersen01} so such conflicts can be easily resolved, while other work aimed at quantifying the degree of which inconsistency arises in KBs \cite{muino11}. Note that consistency does not imply correctness, a KB can be consistent but store factually incorrect information. Similarly a LM can have an incorrect belief about a certain fact but that belief is consistent across different queries.

% \paragraph{Predictability}
% The prediction from existing KBs are predictable in the sense that given a relation triplet (\texttt{Albert Einstein}, \texttt{born-in}, \textbf{X}), the assumed answer for \textbf{X} is that of a location related to where \texttt{Albert Einstein} was born.

% \paragraph{Temporality}
% Since LMs are pre-trained on a certain snapshot of data that belong to a specific moment in time, the knowledge it learnt can quickly become outdated (e.g. the population of some country). Thus their performance have been shown to degrade over time \cite{huang-paul-2018-examining, huang-paul-2019-neural-temporality, lukes-sogaard-2018-sentiment, jaidka-etal-2018-diachronic, floriohatespeech2020}. On the other hand, KBs are designed in a way that ensures any outdated information can be quickly updated to be correct. Since knowledge changes so rapidly, LMs that can update its beliefs automatically and easily are ideal.

% % Given a relation triplet that was valid for several years, such as $\langle$ \texttt{Cristiano Ronaldo}, \texttt{PlaysFor}, \textbf{X} $\rangle$, where \textbf{X} is \texttt{Real Madrid} a KB would be able to update and make the prediction to instead \texttt{Manchester United}. On the other hand, performance in LMs . 

% \paragraph{Reasoning}


% \paragraph{Causality}

% \paragraph{Interpretability} 

==> Survey_ LMs as KB/3_access.tex <==
\section{Accessing Knowledge}

% - Goal: we have LMs, we want to get the same KB abilities but imbue them in LMs
% - First, figure out what ways LMs access knowledge
% - Take the ways that LMs access data, talk about in what way LMs have been improved upon to imbue more entity/relational data (e.g. storage, pretraining strategies, etc.)

% - Types of knowledge:
% --> Factual
% ====> Entity
% --> Linguistic
% --> Commonsense
% ====> Social
% --> Reasoning
% --> Actionable
% - Make a table for this: types of knowledge, the papers that address the types of knowledge, and potentially the task (or way) in which this knowledge is accessed (an example or explanation)

% LMs have the flexibility to access knowledge latent within parameters in various ways. Because of the success of existing LMs on various downstream tasks, researchers have looked to understand the types of knowledge these models encode and how.

% - Define access as storing knowledge and retrieving knowledge

% To access knowledge in a KB, one must be able to first store the knowledge in some form within the KB, whether that be as a KB triple, or in an unstructured text format, then one must create a method for directly accessing the knowledge. As a result, we initially define the act of accessing knowledge as the combination of storing knowledge and retrieving it.

KBs can simply be accessed by querying for specific entity nodes given the starting node and edge corresponding to the relation. In contrast, it is more difficult for LMs to access for specific pieces of knowledge. However, previous research has shown that LMs have the ability to be efficient few-shot and zero-shot learners, which shows that knowledge learned during pretraining can be potentially accessible by finetuning or prompting \cite{brown2020language}. Specifically, finetuning LMs on downstream tasks has shown to be an effective method to tune and elicit specific knowledge for evaluation  \cite{Radford2018ImprovingLU, dong_NEURIPS2019_c20bb2d9}. On the other hand, \citet{Liu2021PretrainPA} has recently shown that prompting shows promise as an effective method to directly access this knowledge without any additional finetuning. %cleverly engineered prompts.

% during evaluation time, if queried in the right way \cite{Adolphs2021HowTQ, }. 

% as the methods to retrieve the knowledge are not able to directly access the parameters in which the specific knowledge may lie.


% While the creation of large LMs is feasible, from a scalability perspective, it is inefficient. As a result, evaluating existing LMs to be better few-shot or zero-shot learners and improving access to knowledge in LMs is an ongoing research question.

% We assess how LMs can become better at accessing knowledge by compiling research on finetuning and prompting. The existing \textit{pretrain and finetune paradigm}  \textit{Pretrain, prompt, and predict} , 

\subsection{Finetuning}

The knowledge stored in a LM is most often inaccessible to the end-user as compared to a KB. Therefore, to retrieve specific pieces of information from a LM, one prevailing method is to finetune the model on a relevant downstream task (e.g. commonsense question answering) so it can make way for the required knowledge to surface in the output during evaluation. Previous work has shown that most knowledge encoded in a LM are acquired during pretraining, while finetuning just learns an interface to access that acquired knowledge \cite{Da2021AnalyzingCE, wallat_bertnesia_2021}. 



\subsection{Prompting}

% limited in the sense that they cannot be infinitely scaled to store large amounts of knowledge. 

% Yet prior work has shown that, despite this limitation, LMs still have the ability to store and query just as much knowledge as KBs, but only when finetuned on specific prompts

The ever-increasing size of LMs make them expensive to finetune and store in practice, despite some architectural innovations that overcomes some of these challenges \cite{Houlsby2019ParameterEfficientTL}. On the other hand, prompting has emerged as an alternative method to extract the wanted knowledge directly from a LM \cite{qin2021learning}. These prompts are often difficult to craft \cite{Adolphs2021HowTQ, qin2021learning, jiang_how_2020}, and small changes in prompts can result in large performance differences, which can in turn affect consistency (see Section \ref{sec:consistency}). Research following the \textit{pretrain, prompt, and predict} paradigm \cite{Liu2021PretrainPA} utilize prompts to induce more knowledge from LMs \cite{petroni_language_2019, davison-etal-2019-commonsense, jiang_how_2020}. Prompting can be divided up into several categories, including \textbf{Discrete Prompts} and \textbf{Soft Prompts}.

% Once prompting is done, LMs can become better few-shot and zero-shot learners \cite{brown2020language}.

\paragraph{Discrete Prompts}
Prompting often enables LMs to learn a specific subtask without extensive finetuning. This paradigm gives the model a familiar query format, which in turn leads to better responses. Many papers tackle prompting from the view of cloze-style like in \citet{petroni_language_2019, davison-etal-2019-commonsense, jiang_how_2020, talmor_olmpics_2020, dhingra_time-aware_2021, liu2021probing} in which these works use prompting to extract specific knowledge, such as commonsense \cite{davison-etal-2019-commonsense}, temporal \cite{dhingra_time-aware_2021, liu2021probing} and factual \cite{petroni_language_2019}, in a format known as \textit{Discrete Prompts}. Prompting has also been applied to specific domains, such as biomedical, to extract domain-specific knowledge \cite{sung2021language}. It was first introduced in \citet{Radford2018ImprovingLU, Radford2019LanguageMA} where it was shown that it could achieve decent zero-shot performance by crafting the right prompt. Knowing that prompting worked well, the same knowledge was applied to smaller LMs. \citet{schick2021exploiting, schick2021its, gao2021making} find that prompting smaller LMs improves performance, especially over supervised baselines. Others also take advantage of this improved performance and evaluate other discrete prompting approaches, such as through entailment \cite{wang2021entailment} and label token optimization \cite{Zhang2021DifferentiablePM}.

The challenge of crafting the ideal prompt for specific task is a non-trivial one. \citet{shin2020autoprompt} tackles this by taking a gradient-based search to find the appropriate prompt for a specific task. \AP creates a template automatically to do so. On the other hand, \citet{LoganIV2021CuttingDO} takes a more manual approach to crafting prompts with comparable accuracy to manual prompts by creating \textit{null prompts}, those of which are task-agnostic and are a simple concatenation of the input and a \texttt{[MASK]} token.

% Despite recent progress in probing for different types of knowledge, these models are still brittle. \citet{kassner2020negated} show that negated factual queries are not easily understood by LMs. Similar to capturing factual knowledge, these LMs also have difficulties capturing commonsense knowledge, such as numerical \cite{lin2020birds} due to biases latent in the the words attended over. To remedy issues regarding capturing knowledge, \citet{Petroni2020HowCA} find that including context of knowledge dramatically improves performance, so similar approaches can be taken to improve upon current limitations in LMs.

\paragraph{Soft Prompts}
Other approaches fall under the categorization of \textit{Soft Prompts}. Those are prompts that are represented by continuous word vectors, used as input and tuned, while keeping the remainder of the model unchanged. \citet{li2021prefixtuning} achieve comparable results on generation while using very few of the model's actual parameters by proposing prefix-tuning; task-specific vectors that can be tuned. Meanwhile, specific to extracting factual knowledge, \citet{qin2021learning, zhong2021factual} find that \textit{Soft Prompts} carry an advantage over \textit{Discrete Prompts} since they are more expressive and can represent multiple contexts simultaneously. \citet{zhong2021factual} takes a gradient-based approach to soft prompting while \citet{qin2021learning} improves upon \AP via continuous word vectors. A number of papers show that soft prompting, when optimized for specific tasks such as relation extraction and natural language understanding, can achieve better performance with minimal tuning \cite{lester2021power, han2021ptr}.

Other methods have been used without editing model parameters. First introduced with GPT-3 \citet{brown2020language}, \textbf{in-context learning}, which adds extra information to the model in the form of in-context demonstrations can improve performance. However, these works are still far from achieving human-level performance \cite{gao2021making, liu2021makes}. 

% Although prompting can improve downstream performance on tasks, the way we query for results can also lead to security and privacy issues. \citet{carlini_extracting_2021} show the consequence of a training data leakage, where private information can be revealed to an attacker. Therefore, care is needed when evaluating methods for prompting and querying data.

% \paragraph{Mining}

% \paragraph{Attacks}

% and through data mining \cite{jiang_how_2020, west_symbolic_2021} and attacking \cite{carlini_extracting_2021}


% Existing research on LMs address accessing knowledge via several strategies, some of which are included in \citet{safavi2021relational}. Namely, this research has explored pretraining on entities and relations \cite{entities-as-experts,facts-as-experts, sun_opql,dejong2021mention} to capture latent representations of entites from structured and unstructured text, augmenting existing models with external parametric memory \cite{yogatama_adaptive_2021,dejong2021mention}, and continual learning \cite{jang_towards_2021} have become the de facto strategies. In the context of the types of knowledge available for LMs, we compare these strategies to understand what current work have tried and what we can further extend and improve on.


% However, what types of knowledge do these LMs often possess? Previously, many existing works focused on evaluating LMs for linguistic knowledge \cite{belinkov-etal-2020-interpretability, hewitt_designing_2019, hewitt-manning-2019-structural, pimentel2020informationtheoretic}. Newer works often investigates whether existing LMs can possess factual \textit{factual} \cite{petroni_language_2019}, \textit{commonsense} \cite{davison-etal-2019-commonsense} , \textit{reasoning} \cite{talmor_olmpics_2020}   knowledge within its parameters. Although there are a plethora of types of knowledge that these LMs might possess, capturing the knowledge in a straightforward and interpretable manner is difficult.

% There are two schools of thought in ways that LMs would be used to gather knowledge. A LM could be prompted for an answer, much like an answer would be mined from a KG, through data mining means. Or, these LMs are analyzed using methods such as probing to understand what these LMs actually know. As a result, we further categorize retrieval methods into two categories: probing for analysis, and extracting knowldge.


==> Survey_ LMs as KB/4_edit.tex <==
\section{Model Editing}

There have been a number of works that address the problem of model editing, with strategies ranging from simple finetuning to making use of an external memory for adding or replacing factual knowledge. To that end, \citet{de_cao_editing_2021} describe a set of rules that editing methods should conform to: \textbf{Generality} implies that the editing method should be capable of changing the facts of \emph{any} LM that is not specifically trained on adaptability. For example, training using meta-learning is one way to make the models editable using a few gradient steps \cite{Finn2017ModelAgnosticMF}. \textbf{Reliability} means that editing a LM should only affect the targeted fact while retaining other unrelated information. \textbf{Consistency} signifies that changes should be consistent across semantically equivalent inputs. \citet{hase_language_2021} measure consistency under entailment (i.e. changing one fact must change other entailed facts in the LM), which \citet{mitchell_fast_2021} call the equivalence neighborhood.   

\subsection{Task Formulation}

To put it formally, given a LM $f_{\theta}$ that contains a collection of implicit factual knowledge $\mathcal{F}: \{(x, y)_i\}$ in its parameters $\theta$ by mapping an input $x_i$ to a potentially undesired output $y_i$, the goal is to obtain a new parameter set $\theta^*$ that conforms to a dataset of revisions $\mathcal{D}: \{(x,\hat{y})_j\}$ by predicting the desired output $\hat{y}_j$ for $x_j$. In addition, the new model $f_{\theta^*}$ should alter the base model's output on the equivalence neighborhood $\mathcal{P}^{x}$ of inputs in $\mathcal{D}$ (i.e. related input/output pairs such as paraphrases of $x$) while leaving the model's behavior intact on other unrelated inputs $\mathcal{O}^{x}$.

\subsection{Finetuning}

\paragraph{Baseline Methods}
One natural strategy to solve this problem is to finetune the model in question or retrain it from scratch on a modified training corpora that is consistent with the new facts. However, such a method would be expensive and impractical for modifying a few datapoints, especially for large LMs. Another approach is to construct a collection of supporting evidences for the modified facts and use it to finetune the model by minimizing a per-instance loss. This method can achieve high performance on the modified facts $\mathcal{D}$, but can significantly degrade the model's performance on the unmodified facts \cite{zhu_modifying_2020}. To obtain a reasonable accuracy on both, one can include evidences from $\mathcal{D}$ and the set of facts that should not be modified $\mathcal{O}^{x}$ in every iteration while finetuning. However, as discussed below, further tricks need to be employed to retain the accuracy on the unmodified facts to avoid catastrophic forgetting. 

\paragraph{Constrained Finetuning} \citet{zhu_modifying_2020} tackle this problem by enforcing a norm-based constraint on the model's weights $\theta$ while finetuning the model on the dataset of revisions $\mathcal{D}$ such that it minimally interferes with the facts that should not be modified. However, such a constraint on the parameter space ignores the highly non-linear nature of LMs \cite{de_cao_editing_2021}. 

\subsection{Hyper Networks}

Another class of methods uses a set of small neural networks (also known as a hyper-networks or learned optimizers) that learns to predict the shift in weights for editing a targeted fact \cite{HyperNetworks}. Specifically, \citet{de_cao_editing_2021} propose \KE that additionally applies a constraint on the update in the function space as opposed to the parameter space like in \citet{zhu_modifying_2020}. The intuition behind this is to predict identical output distributions to the original one for all unrelated inputs $\mathcal{O}^x$. However, this method fails when editing very large models. Therefore, to scale to larger models, \citet{mitchell_fast_2021} propose Model Editing Networks with Gradient Decomposition (\newterm{MEND}) that trains hyper-networks on the standard finetuning gradient of a given correction. The trick they employ is decomposing the gradient into its rank-one outer product form to learn a function $g$ that scales nicely with a model's dimensionality, making it much less computationally expensive than prior methods. In a parallel line of work, \citet{hase_language_2021} introduce a training objective for Sequential, Local, and Generalizing model updates (\newterm{SLAG}). They show that SLAG outperforms previous methods when updating multiple beliefs in sequence.

\subsection{Direct Editing}

\citet{meng2022locating} propose another method they call Rank-One Model Editing (\newterm{ROME}) for modifying factual knowledge in large neural networks. Specifically, they consider the transformer MLP modules as simple key-value memories \cite{geva2021transformer}, and editing a specific fact is just a matter of locating the relevant MLP weights by causal tracing then writing to it directly the new key-value pair using a rank-one modification.   


% \subsection{Constrained Finetuning} 

% \citet{zhu_modifying_2020} tackles this problem by enforcing a constraint on the model's weights $\theta$ while finetuning it on the dataset of revisions $\mathcal{D}$ such that it minimally interferes with the facts that shouldn't be modified. This is done by subjecting the parameters to the following constraint: $||\theta - \theta_0|| \leq \delta$ where $\theta_0$ are the initial parameters, $\delta$ is a small positive constant and $|| \cdot ||$ is the $\ell_\infty$ norm as it has been shown to lead to more stable result as compared to other norms \cite{zhu_modifying_2020}. Further, the authors found that finetuning only the first and last Transformer blocks results in better adaptation to the modified facts while preserving knowledge on the other unrelated facts. However, such norm-based constraint ignores the highly non-linear nature of LMs, since a minimal change in parameter space may result in different output for many other datapoints \cite{de_cao_editing_2021}. 

% \subsection{Hyper-networks} 

% This class of methods uses a small neural network (also known as a hyper-network) that learns to generate the weights of another network \cite{HyperNetworks}. Several works have employed this strategy to edit the parameters of a LM.

% \paragraph{\KE}
% \citet{de_cao_editing_2021} propose a method that casts the learning task as a constrained optimization problem. Specifically, a hyper-network $g$ parameterized by $\phi$ is used to predict the shift $\Delta\theta$ in weights rather than the final parameters directly. Thus the updated parameters will be $\theta' = \theta + g(x,y,\hat{y}; \phi)$ and the constraint on the update will be in terms of sums of Kullback-Leibler (\newterm{KL}) divergences from the updated model to the original one in the function-space as opposed to the parameter-space like \cite{zhu_modifying_2020}. The intuition behind this constraint is to predict identical output distributions to the original one for all unrelated inputs $\mathcal{O}^x$. In order to make it tractable, they approximate this constraint via Monte Carlo (\newterm{MC}) sampling or by evaluating on a subset of the sample space via beam search. However, \KE have been shown to fail when it comes to editing very large models.

% \paragraph{MEND} 
% To scale to larger models, \citet{mitchell_fast_2021} introduce Model Editing Networks with Gradient Decomposition (\newterm{MEND}). It works by training a set of lightweight hyper-networks on the standard finetuning gradient of a given correction. The trick they employ is decomposing the gradient into its rank-1 outer product form to learn a function $g$ that scales nicely with a model's dimensionality, making it much less computationally expensive than prior methods. 

==> Survey_ LMs as KB/5_consistency.tex <==
\section{Consistency}
\label{sec:consistency}

% In this paper, we consider consistency in light of five different contexts: (1) Paraphrasing, where a LM should provide the same answer when asked for the same fact but under a different wording. (2) Reasoning, implies that a LM is capable of reasoning consistently over both explicit input statements and implicit knowledge encoded in the parameters of the network. (3) Causality, ... (4) Fact-Checking, ... (5) Multilinguality, is the same as paraphrases, where a multilingual model should respond similarly to the same sentence but expressed in a different language. 


LMs are shown to suffer from a lack of consistency in their answers \cite{elazar_measuring_2021}. For example, they can provide different results when queried for the same fact but under a different wording (i.e. a paraphrase). In this section, we consider consistency in light of three different contexts: \textbf{Paraphrasing}, \textbf{Commonsense} and \textbf{Multilinguality}.

\paragraph{Paraphrase}
\citet{bhagat13} define the term \textit{quasi-paraphrases} as `sentences or phrases that convey approximately the same meaning using different words'. The word \textit{approximately} is key here, since it does not assume the strict and logical equivalence of paraphrase. This fuzzy definition allows for a broader set of samples to be considered as paraphrases, and is of interest when considering consistency for LMs. Therefore, one method for measuring the consistency of a model is to probe it using paraphrases of the same relation for a specific subject, and test whether it always predicts the same object or not \cite{kassner2020negated, Ettinger20, elazar_measuring_2021}. To that end, several benchmarks have been proposed to measure consistency of LMs \cite{ravichander-etal-2020-systematicity, elazar_measuring_2021}, while other datasets have been adapted for that purpose \cite{levy-etal-2017-zero, wang2021}. For instance, \citet{de_cao_editing_2021} and \citet{mitchell_fast_2021} employ back-translation to generate paraphrases \cite{sennrich-etal-2016-improving, wieting-gimpel-2018-paranmt} for measuring consistency after editing factual knowledge in LMs. To mitigate this lack of consistency, \citet{elazar_measuring_2021} include a new term in their loss function that aims to minimize the Kullback-Leibler (\newterm{KL}) divergence for instance between the output distribution of different paraphrases.

% previous work have included a new term in their loss function that aims to minimize the Kullback-Leibler (\newterm{KL}) divergence for instance between the output distributions of different paraphrases \cite{elazar_measuring_2021}. 

\paragraph{Commonsense}
Consistency, however, is not limited to paraphrasing. Previous work explores the brittleness of LMs and the addition of a negation element (e.g. not) to a probe \cite{kassner2020negated, Ettinger20}. Specifically, a LM can maintain two contradictory beliefs in its parameters, such as ``\texttt{Birds can fly}'' and ``\texttt{Birds cannot fly}'', showing that they are insensitive to the contextual impacts of negation. Further, \citet{kassner2020negated} show an equal effect when mispriming the probe with a misleading distractor (e.g. \texttt{Talk? Birds can [MASK]}). Robust LMs will not only be consistent under different paraphrases and negations, but also under entailment. \citet{hase_language_2021} measure consistency under entailment, including contrapositives, after updating beliefs of a LM. Specifically, they adapt the LeapOfThought dataset \cite{talmor_leap--thought_2020} such that each datapoint has a main fact (e.g. \texttt{A viper is a vertebrate}) that they update and an entailed claim (e.g. \texttt{A viper has a brain}) that they check the truth value of with respect to the model's updated beliefs. Similar to the efforts done for overcoming lack of consistency under different paraphrases, \citet{hase_language_2021} add another loss term to their objective function to minimize the error across entailed data. On the other hand, \citet{kassner_beliefbank_2021} use a feedback mechanism that issues relevant information from a symbolic memory of beliefs as input to the system during test-time in order to improve consistency under entailment. 
 

\paragraph{Multilingual}
Crosslingual LMs that are trained on several languages, such as XGLM \cite{Lin2021FewshotLW}, must be consistent across the languages they support. For example, the same probe queried in different languages must provide the same fact. \citet{liu_knowledge_2021} design a knowledge-based multilingual LM pretraining framework using Wikidata \cite{wikidata} that shows improvement on crosslingual NLP tasks, but neither they nor other work measure consistency under multilinguality.

==> Survey_ LMs as KB/6_reasoning.tex <==
\section{Reasoning}

% \input{tables/reasoning_table}

It has been a long-standing goal of AI to reason over explicit knowledge given to it in order to reach conclusions \cite{McCarthy_Programs59, NewellLogic56, Metaxiotis2002ExpertSI}. The advent of LMs has brought this dream closer to reality \cite{Clark2020TransformersAS}. Concretely, LMs are shown to leverage the knowledge they learn during pretraining to perform well on reasoning tasks expressed in natural language rather than in formal representations. Such tasks include: commonsense \cite{Da2021AnalyzingCE}, natural language inference \cite{bowman-etal-2015-large}, mathematical \cite{Saxton2019AnalysingMR, Polu2022FormalMS}, rule-based \cite{Clark2020TransformersAS}, inductive \cite{Misra2021OnSC} and abductive reasoning \cite{Bhagavatula2020AbductiveCR}. However, we focus on types of reasoning that KBs have been shown to perform better on NLP tasks.

\subsection{Symbolic Reasoning}

\paragraph{Logical Reasoning} 
Previous work show that LMs can perform rule-based reasoning by emulating the process of binding facts with low level first order logic rules to deduce a conclusion \cite{Clark2020TransformersAS, talmor_leap--thought_2020, Gontier2020MeasuringSG}. LMs can also generate proofs demonstrating their `chain of thought' \cite{Saha2020PRoverPG, tafjord-etal-2021-proofwriter, Polu2022FormalMS}. \citet{Wei2022ChainOT} show that inducing a prompt that mimics the reasoning process improves the performance on reasoning tasks such as math word problems.

\paragraph{Mathematical Reasoning}
In another line of work, \citet{Nye2021ShowYW} show that LMs can perform complex multi-step computations when asked to generate the results of intermediate steps. \citet{Polu2022FormalMS} show that by using expert iteration (i.e. proof search \cite{Polu2020GenerativeLM} interleaved with curriculum learning) a LM can solve complex mathematical problems.  

\paragraph{Limitations}
Despite these successes, the best models are still unable to chain more than 2 or 3 non-trivial steps of complex reasoning \cite{Polu2022FormalMS}. Further, it largely remains an open question of whether the LMs are indeed ``reasoning'' or just emulating the thought process of humans \cite{Wei2022ChainOT}. 

\subsection{Commonsense Reasoning}
Commonsense reasoning is the ability to reason about the underlying nature of situations humans encounter on a day-to-day basis such as the effects of Newtonian physics and the intentions of others. LMs are shown to possess a certain amount of commonsense knowledge in their parameters \cite{petroni_language_2019, davison-etal-2019-commonsense, Zhou_Zhang_Cui_Huang_2020, cui-etal-2021-commonsense}. As a result,  \citet{huang-etal-2019-cosmos, talmor-etal-2019-commonsenseqa, sap2019atomic, west_symbolic_2021} introduce datasets to evaluate the extent to which LMs can reason over the knowledge they learned during pretraining.
In addition to implicit reasoning, \citet{talmor_leap--thought_2020} show a way in which LMs can systematically reason over both explicit input statements given to the model by a user and the implicit knowledge stored in the parameters of the model. However, despite succeeding in commonsense leaderboards, \citet{Merrill2021ProvableLO} suggest that those models fail to understand the underlying semantics leading them to commit trivial mistakes.


% Symbolic reasoning involves manipulating mathematical and logical rules to come to a conclusion. Since following the train of thought through a KB is simpler than that of an LM, existing work has approached understanding how LMs symbolically reason. 
% As a result, several datasets have emerged to evaluate the extent to which LMs can reason over the knowledge it learned during pretraining \cite{huang-etal-2019-cosmos, talmor-etal-2019-commonsenseqa, sap2019atomic, west_symbolic_2021}.














==> Survey_ LMs as KB/7_explainability.tex <==
\section{Explainability \& Interpretability}
While the field of NLP has traditionally been guarded by the use of inherently explainable and interpretable techniques, the move from predominantly statistical NLP methods to black box neural models have only motivated the necessity to return to the study of explainability and interpretability.

While literature in NLP and computer science combine explainability and interpretability as similar, if not, identical aspects \cite{dosilovic_explainable_2018}, we aim to clarify these confusions by creating clear definitions for both terms. In short, we define \textbf{Interpretability} as the inspection of the inner workings of the model and understanding the reasoning behind model predictions by evaluating internal mechanisms. On the other hand, \textbf{Explainability} is a focus on the outward appearance of a model, namely whether the model's outputs are explainable in a post-hoc setting.

Since our main goal is to apply these \lmkb in practice, LMs that are not explainable and interpretable are often undeployable. For example, prior work has identified that BERT \cite{devlin-etal-2019-bert}, while powerful, is inherently opaque with respect to its inner workings \cite{rogers_primer_2020}. KBs, on the other hand, are far easier to read, as their fixed schemas are simpler to interpret. Having the same level of explainability inherent in LMs as we do in KBs would vastly improve their practical use. However, while KBs are naturally explainable, they do not inherently have interpretable qualities. So we make the distinction that, while we talk about both aspects with respect to LMs, we in tangent explain interpretability to cover all aspects of explainable AI in LMs.

\subsection{Interpretability}
Transformer models \cite{vaswani17attention, devlin-etal-2019-bert, Liu2019RoBERTa, Raffel2020ExploringTL} are composed of different building blocks: the encoder, decoder, self-attention, and more. However, we know little of how these building blocks work. Even as newer LMs are devised, some model capabilities remain uninterpreted, and problematic behaviors become evident even after a model has been in use for a long period of time. As a result, a deep understanding of the mechanisms that drive these models is imperative for long-term use and applied success in the real world.

\paragraph{Probing} Because little is known about how neural models function, many researchers opt to understand these models via probing. In its most basic form, one type of probing is done by way of the use of a simple linear classifier to associate internal representations with external properties \cite{belinkov-etal-2020-interpretability}. Probing allows researchers to answer questions about how the models function, their structure, or the decisions that these models make, especially regarding how these models learn linguistic structures \cite{tenney2018what,hewitt_designing_2019,hewitt-manning-2019-structural, belinkov-etal-2020-interpretability}.

\paragraph{Attention} With the introduction of attention-based LMs \cite{vaswani17attention}, researchers have attempted to use attention \cite{Bahdanau2015NeuralMT} to interpret the inner workings of the models. However, attention heads have been found to be fairly uninterpretable, as \citet{michel2019sixteen} has found that multiple attention heads have little impact on performance. Other transformer-based attention research has evaluated whether these models actually learn linguistic and syntactic structure and the relationship between them \cite{tenney2019bert, jawahar-etal-2019-bert, clark2019does, vig2019analyzing}.

% For example, attention heads have been found to be fairly uninterpretable, as \citet{michel2019sixteen} has found that multiple attention heads have little impact on performance.

% Past work has evaluated and improved the explainability of attention through sparsity of 

However, many previous works have also contended whether attention can convey proper explanations \cite{jain2019attention, serrano2019attention, wiegreffe2019attention}. \citet{jain2019attention} and \citet{serrano2019attention} argue that attention cannot be used as a \textit{faithful} explanation for the model. On the other hand, \citet{wiegreffe2019attention} contradicts both statements by noting that there is a \textit{plausible} chance that attention could be correlated with the model. However, this claim is dependent on one's definition of explanation. \citet{mohankumar2020transparent} follows up prior work to note that the distribution of attention fails to fall on important words and strays to unimportant tokens. As a result, the definition of whether attention can adequately provide an explanation for the inner workings of LMs remains opaque. 

\paragraph{Transformer Mechanisms} We evaluate transformers and whether they are explainable via other mechanisms, such as the feedfoward layers \cite{zhao2021nonlinearity, geva2021transformer, meng2022locating}. \citet{zhao2021nonlinearity} propose a tool to measure non-linearities in LMs by taking into account geometry space of embeddings, finding that the non-linearity of the self-attention feedforward layers and MLPs of a LM follow similar patterns, but their functions are less known. \citet{geva2021transformer} extrapolate from this learned fact and find that feedforward layers in LMs are just key value memories; as a result \citet{meng2022locating} are able to use their method of causal tracing to locate the knowledge and use the key value pairs to access knowledge within the feedforward layers and make modifications to it.

\paragraph{Mechanistic Interpretability} Akin to reverse engineering software, if we could reverse engineer transformers, we could garner more understanding about the inner workings of these models. \citet{elhage2021mathematical} introduces mathematical conception as a way to understand the internal operations within. In addition, they also discover that attention heads can explain in-context learning within smaller models. Their promising results highlight the potential for further development of mathematical tools to understand computational patterns.

\paragraph{Causal tracing} Introduced in \citet{meng2022locating}, causal tracing is another form of accessing in which the model is traced for the path of information within. To do so, the model is run multiple times while corruptions are introduced to the system, then the system is restored to tease out which changes restored the original results. Their results show that it is possible to identify activations that are related to a model's factual predictions.

\subsection{Explainability}
The more we better explain the output of existing LMs, the better we can tailor these systems to real-world use. These explanations for model behavior could in turn be used to correct model shortcomings and improve help the end user gain trust in a system.

\paragraph{Influence Functions} One way to explain a black box model is through a technique known as an influence function. First introduced by \citet{hampel1974}, \citet{koh2020understanding} applies influence functions to neural models by using second-order optimization techniques; presenting a method that enable influence functions to be used to interpret model outputs.

\citet{han2020explaining} applies influence functions to LMs, finding that influence functions may be better suited for more complex tasks, such as natural language inference, despite these methods being computationally prohibitive \cite{pezeshkpour2021empirical}. Gradient-based and non-Hessian information \textit{influence attribution} methods \cite{pezeshkpour2021empirical} have been introduced to speed up computation. \cite{pezeshkpour2021combining} also introduce the combination of influence atrtibution with saliency maps to find artifacts in training data more accurately than using influence functions alone.

Influence functions have also been used for interactive debugging by way of using humans as feedback after interpreting their output \cite{zylberajch-etal-2021-hildif}. In this way, we show promise that there is a potential to integrate these explainability tools with humans in a more practical setting.

\paragraph{Explanations}
Researchers have introduced the potential for LMs to generate coherent explanations of their decisions. LMs such as T5 \cite{Raffel2020ExploringTL} are able to generate explanations that achieve state-of-the-art performance on explainability benchmarks \cite{Narang2020WT5TT}. Despite the push to use explanations as a way to improve explainability within LMs, these explanations are still inconsistent and fickle. \citet{Camburu2020MakeUY} show that by using an adversarial framework to interject modified inputs, they are able to show that LMs generate a large number of inconsistencies in their explanations.

Other methods have shown that LMs can learn to generate the reasoning process behind their decisions using prototype networks \cite{Schramowski21}, through highlighting fragments of the input text to justify the output \cite{Lei2016RationalizingNP}, or using human-provided explanations in the training process \cite{Camburu2018eSNLINL, paranjape-etal-2021-prompting}.

==> Survey_ LMs as KB/8_models.tex <==
\section{Models}
\input{tables/models}


In the previous sections, we detail more general aspects of LMs. In this section, we cover the different models that fall under the \lmkb paradigm and the solutions proposed by these models that improve LM performance.

These models often incorporate knowledge explicitly through several means: via some form of \textbf{pretraining} strategy that explicitly encodes entity-level or relation-level data or via the integration of \textbf{external memory} to an existing LM. Models that implicitly contain knowledge, such as existing pretrained LMs, are not covered in this section, as we focus on explicit incorporation of knowledge.



% - external memory
% --> via external knowledge graphs
% --> via parametric memory
% --> via additional attention mechanisms?

% - pretraining
% --> pretraining on entities
% --> pretraining on relations
% --> pretraining on ???

\subsection{External Memory} Existing LMs are often unable to store localized information about facts and specific knowledge; on the other hand, KBs have been known to store information about millions of entities. Knowing this, existing research has focused on taking advantage of the storage capabilities of existing KBs and integrating this capability into LMs \cite{wei2021knowledge}.

\citet{heinzerling_language_2021} introduced initial work understanding how \lmkb can be used in more general settings, especially in integrating knowledge about general and rare entities, since representing millions of entities within LMs is difficult when LMs have a limited vocabulary. Current work often forgoes the potential to deploy these \lmkb in the real world. To improve existing LM and overcome memory limitations, current work has focused on the goal of improving memory for LMs to store more information about external information, such as information about entities in a sentence.

External memory has previously been used for neural networks \cite{Bahdanau2015NeuralMT, weston2015memory, graves2014neural, ahn2017neural}. \citet{ahn2017neural} specifically proposed the \newterm{Neural Knowledge Language Model} (NKLM) to take advantage of external knowledge and exploit factual knowledge. Since then, a large number of works have focused on the integration of this external memory to improve performance on knowledge-intensive tasks. To summarize these works, we focus on detailing the different strategies of integrating external memory within LMs and how they can be further improved on.

\subsubsection{External Knowledge Graphs}
Much work prior to the focus on \lmkb focus on the integration of KBs explicitly within LMs. Thus, Knowledge Enhanced Pretrained LMs \newterm{KE-PLM} \cite{wei2021knowledge} have become the backbone of models that integrate knowledge explicitly. 

External knowledge graphs (KGs) have been known to 

\subsubsection{Parametric, Semiparametric, and Non-Parametric Memory}
We focus on parametric, semi-parametric, and non-parametric memories integrated within LMs. \textbf{Parametric memory} can be seen as memory latent within LMs; \textbf{non-parametric memory} can be seen as memory that is used in addition to internal LM memory; and \textbf{semiparametric memory} can be seen as a combination of both parametric memory and non-parametric memory.

\paragraph{Parametric Memory}

\paragraph{Non-Parametric Memory}

\paragraph{Semiparametric Memory} \citet{yogatama_adaptive_2021} introduce the idea of semiparametric memory.

\subsubsection{Attention over Memory}


\subsection{Pretraining}
Models have been known to encode knowledge within their parameters through unsupervised methods, specifically pretraining. For example, given the example \texttt{Obama is from [MASK]}, using a masked language modeling (MLM) objective, we would expect the model to predict \texttt{Hawaii}. However, there is no explicit integration of any entity-level or relation-level knowledge through this objective. As a result, a number of works have sought to incorporate entity-level or relation-level knowledge through pretraining strategies and loss function modifications. 

==> Survey_ LMs as KB/8_tasks.tex <==
\section{Tasks}
As a starting point, we detail the different tasks and models that have been designed to get closer to the goal of \lmkb. One challenge of this is the fact that there does not currently exist standardized benchmarks for \lmkb, likely owing to the fact that knowledge latent within LMs can be measured in a multitude of tasks. However, our goal is to delineate a set of tasks that can be used initially as measurements to achieve this goal.



==> Survey_ LMs as KB/9_limitations.tex <==
\section{Future Work \& Limitations}

In this paper, we review the literature with respect to five aspects that LMs need to be proficient at to qualify as KBs. However, despite these recent breakthroughs, the community still has a long way to go to enable the real-world deployment of LMs. For instance, pretrained LMs need explicit tuning on a consistency corpus \cite{elazar_measuring_2021} in order to behave similarly under different paraphrases. They are also sensitive to word-order, negation, priming, and patterns \cite{kassner2020negated} and are unreliable out-of-the-box. Furthermore, previous work demonstrates that there are theoretical limitations to transformers that prevents them from performing certain types of reasoning tasks \cite{hahn-2020-theoretical, Bhattamishra2020OnTP, helwe2021reasoning}. They also lack social intelligence \cite{Liang2021TowardsUA}, an understanding of time \cite{dhingra_time-aware_2021, lazaridou_mind_2021}, causality \cite{Li2021CausalBERTIC}, dealing with uncommon facts \cite{poerner-etal-2020-e, jiang-etal-2020-x} and counterfactual reasoning \cite{Feng2021EmpoweringLU}. We hope that by uncovering the limitations of LMs from the perspective of KBs, we can continue to motivate exploring intrinsically the positives of KBs and apply the knowledge to improving LMs.


==> Survey_ LMs as KB/a_models.tex <==
\section{Models}
% Talk about external KBs+LMs, then talk about LMs-as-KBs, then continue to talk about things like parametric memory and external memory and pretraining'

\input{tables/models}

In the main sections, we detail more general aspects of LMs. To follow the sections, we cover the different models that fall under the \lmkb paradigm and the solutions proposed by these models that improve LM performance.

These models often incorporate knowledge explicitly through a combination of several means: via some form of \textbf{pretraining} strategy that explicitly encodes entity-level or relation-level data, via the integration of \textbf{external memory} to an existing LM, via an \textbf{attention-based mechanism}, or via a \textbf{retrieval-based} model that gathers the appropriate nodes of a KG. Models that implicitly contain knowledge, such as existing pretrained LMs, are not covered in this section, as we focus on explicit incorporation of knowledge.

\subsection{External Memory} Existing LMs are often unable to store localized information about facts and specific knowledge; on the other hand, KBs have been known to store information about millions of entities in an interpretable fashion. Knowing this, existing research focus on taking advantage of the storage capabilities of KBs and integrating this capability into LMs \cite{wei2021knowledge}.

\citet{heinzerling_language_2021} introduce initial work understanding how \lmkb can be used in more general settings, especially in integrating knowledge about general and rare entities, since representing millions of entities within LMs is difficult when LMs have a limited vocabulary. Recent work often forgo the potential to deploy these \lmkb in the real world. To improve existing LM and overcome memory limitations, recent work focuses on the goal of improving memory for LMs to store more information about external information, such as information about entities in a sentence.

External memory has previously been used for neural networks \cite{Bahdanau2015NeuralMT, weston2015memory, graves2014neural, ahn2017neural}. \citet{ahn2017neural} specifically propose the \newterm{NKLM} to take advantage of external knowledge and exploit factual knowledge. Now, a large number of works now integrate external memory to improve performance on knowledge-intensive tasks. To summarize these works, we focus on detailing the different strategies of integrating external memory within LMs and how they can be further improved on.

\subsubsection{External Knowledge Graphs}
\label{app:kgs}

% Much of the work prior that focuses on \lmkb involves external knowledge graphs (KG): either the creation of the KGs or the integration of the KGs into models, exploring the potential for commonsense KGs, 

% Much of the prior work on \lmkb involves the explicit creation of external knowledge graphs (KG) that are incorporated into models, such as in the work \newterm{COMET} \cite{bosselut2019comet}. COMET explores the potential for transformers \cite{vaswani17attention} to be used for knowledge graph completion, outputting knowledge base triples in a structured manner. This shows that innately, these models had the ability to create structured knowledge. 

Prior work on \lmkb involves the explicit creation of external knowledge graphs (KG) that are incorporated into models, such as in the model \newterm{KGLM} \cite{logan2019baracks}. KGLM looks at explicitly incorporating KGs into LMs. KGLM can access facts which are stored in a KG, growing constantly as new facts are added. The model selectively grows the KG if a fact is not there or refers back to the KG to pick an existing fact.


While not explicitly a model, \newterm{GRF} \cite{ji2020language} propose a method to enable multi-hop reasoning with transformers. To do so, the model first encodes multi-relational graphs to obtain representations for concepts, then reasons over multiple relational paths to generate the concept, and finally chooses the output by determining the probability of obtaining the concept from the KG versus choosing a word from its innate vocabulary.

Other work also evaluate other domains. \citet{he-etal-2020-bert} introduce \newterm{BERT-MK}, which integrates contextualized knowledge from a medical KG, which shows improvement over existing biomedical models on entity typing and relation classification tasks.

% Much work prior to the focus on \lmkb focus on the integration of KBs explicitly within LMs. Thus, Knowledge Enhanced Pretrained LMs \newterm{KE-PLM} \cite{wei2021knowledge} have become the backbone of models that integrate knowledge explicitly. 

% External knowledge graphs (KGs) have been known to 

\subsubsection{Non-parametric Memory}
Non-parametric memory can be seen as memory that is used in addition to internal LM memory. Existing work integrates non-parametric memory with LMs to improve performance on downstream tasks.

\citet{ahn2017neural} adapts an early version of non-parametric memory with neural models using \newterm{NKLM}. NKLM is able to combine
symbolic knowledge provided from a KG with an RNN \cite{hochreiter1997long}.

Other work adopt a similar strategy via embeddings to incorporate entity knowledge. Early work on \newterm{KnowBERT} \cite{peters2019knowledge} introduces entity vectors that are computed from mention-span representations that are obtained from BERT \cite{devlin-etal-2019-bert} to form entity-span representations. Other work follow similarly: \citet{Fvry2020EntitiesAE} introduce \newterm{EAE}, a LM augmented with entity memory to keep track of facts about entities. Building off of this, \newterm{FAE} \cite{facts-as-experts} adds an additional memory that encodes triples from a symbolic KB that can be accessed with key-value memory to extract facts and improve predictions. Other models such as \newterm{ERNIE}, \newterm{KEPLER}, and \newterm{KALM} use existing algorithms to embed entity and relation knowledge into embeddings \cite{zhang-ernie-2019, Wang2021KEPLERAU, Rosset2020KnowledgeAwareLM}. \newterm{RAG} uses vector indices of Wikipedia to access latent information during inference on knowledge-intensive tasks \cite{lewis_retrieval-augmented_2021}

Introduced by \cite{dhingra2020differentiable},  \newterm{DrKIT} includes a virtual knowledge base (VKB), which is a "soft knowledge base" that is used in conjunction with neural methods to compensate for structure and find answers to questions. \citet{sun_opql} improve the idea of a VKB and introduces an additional strategy to learn entity and information through \newterm{OPQL}, utilizing key-value memory to learn relationships between entities and relations. \citet{dejong2021mention} take the idea of a VKB and insert it into \newterm{TOME} as non-parametric memory to improve reasoning over various knowledge sources.

Episodic non-parametric memory can also be introduced to LMs to remember specific knowledge, including both short-term and long-term contexts \cite{dAutume2019EpisodicMI, yogatama_adaptive_2021, Liu2022RelationalMA}.

\citet{Liu2020KBERTEL} try a different strategy by introducing a visible matrix for their model \newterm{K-BERT} to control the impact of certain knowledge injected.

\subsubsection{Attention over Memory}
Attention mechanisms over specific types of memory can extract salient information during inference. Early iterations of attention over memory can be seen in KnowBERT \cite{peters2019knowledge} where they introduce \newterm{KAR}, a form of multi-headed attention between word representations and knowledge-enchanced entity span vectors. On the other hand, in TOME \cite{dejong2021mention}, they employ attention over an entire VKB within a transformer model to retrieve the relevant pieces of knowledge.

Other work modify existing transformer layers to add an additional self-attention mechanisms over entity knowledge, specifically looking at using the attention to identify the query mechanisms required depending on the attending token and token attended to \cite{Yamada2020LUKEDC, Ri2021mLUKETP}.

\subsection{Pretraining}
Models have been known to encode knowledge within their parameters through unsupervised methods during pretraining. For example, given the example \texttt{Obama is from [MASK]}, using a masked language modeling (MLM) objective, we would expect the model to predict \texttt{Hawaii}. However, there is no explicit integration of any entity-level or relation-level knowledge through this objective. As a result, a number of work have sought to incorporate entity-level or relation-level knowledge through pretraining strategies and loss function modifications.

Various models focus on different pretraining strategies, whether that be through the augmentation of the input or modification of loss functions or others. FAE adapts from the the EAE model to introduce a pretraining scheme modeled as a cloze-type Question Answering (QA) task \cite{facts-as-experts}. Other pretraining tasks include an augmentation of the existing masked language modeling (MLM) task by masking the entities and predicting the entities during pretraining \cite{sun_opql, Yamada2020LUKEDC, Ri2021mLUKETP, zhang-ernie-2019} or introducing multiple preexisting pretraining tasks to be used in conjunction with each other, such as MLM \cite{Yamada2020LUKEDC, Ri2021mLUKETP}. \citet{Sun2019ERNIEER} introduce three levels of masking for their pretraining task: basic-level, phrase-level, and entity-level masking. Other work introduce a special loss function in conjunction with the standard MLM objective that focuses on predicting entities \cite{Rosset2020KnowledgeAwareLM}, linking entities to text \cite{entities-as-experts, facts-as-experts, sun_opql, dejong2021mention}, objectives focusing on semantic understanding of relations and entities \cite{Qin2021ERICAIE}, or knowledge embedding objective where entities and relations are encoded in KGs as distributed representations KE \cite{wang_language_2020}.

Some models are trained on inputs augmented specifically to encode better representations of entities and relations. For example, \citet{dejong2021mention} inserts start and end entity tokens around each entity in the input. Others mask both relations and entities during pretraining, like in \citet{sun_opql}. \citet{Yao2019KGBERTBF} also imbues entity and relation information by taking the entities and relations in a sequence as input into existing LMs. 

% Methods to incorporate more knowledge through data not commonly used has been applied in \citet{aghajanyan_htlm_2021, Aghajanyan2022CM3AC}, through unimodal and multimodal settings.
\citet{aghajanyan_htlm_2021, Aghajanyan2022CM3AC} look at methods to incorporate more knowledge with data not commonly used in unimodal and multimodal settings. In \citet{aghajanyan_htlm_2021, Aghajanyan2022CM3AC}, both \newterm{HTLM} and \newterm{CM3} models apply scraped HTML and find that pretraining with size hints and prompting with BART \cite{lewis-etal-2020-bart} can creative effective transfer to a wide range of downstream tasks and supervision levels. These approaches show the potential for web-scrapped data to be used as viable signals for model pretraining on knowledge-intensive tasks.

\subsection{Retrieval}
Some models can capture more knowledge in modular and interpretable ways via retrieval methods. \citet{guu_realm_2020} introduce \newterm{REALM} which contain ways to extract knowledge by applying retrieval-based methods during pretraining, finetuning, and inference. Their method allows retrieval of Wikipedia knowledge and ability for the model to decide what kinds of information to query during inference. \citet{lewis_retrieval-augmented_2021}'s RAG follow the same retrieval-based approach but instead integrates a non-parametric seq2seq to improve on tasks outside of open-domain extractive question answering. In the case of multi-task settings, \citet{Maillard2021MultitaskRF} show that it is indeed possible to develop a universal multi-task retriever using non-task-specific methods using a passage and query encoder shared across all tasks.

==> Survey_ LMs as KB/tables/models.tex <==
\begin{table*}[]
\begin{adjustbox}{width=1\textwidth,center}
\begin{tabular}{llccccc}
\toprule
\textbf{Name}            & \textbf{Author}          & \textbf{External KG} & \textbf{Non-Parametric Memory} & \textbf{Pretraining} & \textbf{Attention} & \textbf{Retrieval} \\ \midrule
QA-GNN        & \citet{yasunaga2021qagnn}   & \checkmark             &                       &             &           &           \\ \hline
KnowBERT        & \citet{peters2019knowledge}    &             &   \checkmark     &  \checkmark           &           &           \\ \hline
KGLM            & \citet{logan2019baracks}   & \checkmark            &                       &             &           &           \\ \hline
NKLM            & \citet{ahn2017neural}        &             &             \checkmark &            &           &           \\ \hline
REALM           & \citet{guu_realm_2020}        &             &                       &             &           & \checkmark           \\ \hline
EAE             & \citet{entities-as-experts}      &             &     \checkmark    &           &           &           \\ \hline
FAE             & \citet{facts-as-experts}      &             &     \checkmark       &   \checkmark            &           &           \\ \hline
OPQL-LM         & \citet{sun_opql}        &             &     \checkmark    & \checkmark              &           &           \\ \hline
TOME            & \citet{dejong2021mention}    &             &     \checkmark        & \checkmark              &  \checkmark         &           \\ \hline
RAG             & \citet{lewis_retrieval-augmented_2021}      &             &    \checkmark                     &             &           &   \checkmark  \\ \hline
LUKE            & \citet{Yamada2020LUKEDC}     &             &                       & \checkmark            &     \checkmark      &           \\ \hline
mLUKE           & \citet{Ri2021mLUKETP}         &             &                       &   \checkmark          &    \checkmark       &           \\ \hline
ERNIE           & \citet{zhang-ernie-2019}      &             &  \checkmark                     &  \checkmark           &           &           \\ \hline
ERICA           & \citet{Qin2021ERICAIE}        &             &                       &  \checkmark           &           &           \\ \hline
KEPLER          & \citet{wang2021}       &             &                       & \checkmark            &      \checkmark     &           \\ \hline
% COMET           & \citet{bosselut2019comet}   & \checkmark            &                       &             &           &           \\ \hline
SPALM           & \citet{yogatama_adaptive_2021}   &             &   \checkmark                    &             &           &           \\ \hline
GRF             & \citet{ji_survey_2021}         & \checkmark            &                       &             &           &           \\ \hline
RelationLM      & \citet{Liu2022RelationalMA}.        &             &   \checkmark                    &             &           &           \\ \hline
HTLM            & \citet{aghajanyan_htlm_2021} &             &                       &  \checkmark           &           &           \\ \hline
CM3             & \citet{Aghajanyan2022CM3AC} &             &                       &  \checkmark           &           &           \\ \hline
K-BERT          & \citet{Liu2020KBERTEL}        &             &   \checkmark                    &             &           &           \\ \hline
ERNIE           & \citet{Sun2019ERNIEER}        &             &                       &  \checkmark           &           &           \\ \hline
KG-BERT         & \citet{Yao2019KGBERTBF}        &             &                       &  \checkmark           &           &           \\ \hline
BERT-MK         & \citet{he-etal-2020-bert}         &   \checkmark          &                       &             &           &           \\ \hline
KALM            & \citet{Rosset2020KnowledgeAwareLM}     &             &    \checkmark                   & \checkmark            &           &           \\ \hline
DrKIT           & \citet{dhingra_time-aware_2021}    &             &                       & \checkmark            &           &           \\ \hline
MBPA++          & \citet{dAutume2019EpisodicMI}   &             &   \checkmark                    &             &           &           \\ \hline
Multitask Model & \citet{Maillard2021MultitaskRF}   &             &                       &             &           &   \checkmark        \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Models and the associated modifications to improve knowledge within their parameters.}
\end{table*}

==> Survey_ LMs as KB/tables/probes.tex <==
\begin{table*}[t]
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcc}
\toprule
\textbf{Task Name} & \textbf{Paper} & \textbf{Examples} \\ 
\midrule
LAMA & Petroni et al. & Obama was born in \textit{[MASK]}, where \textit{[MASK]} = Hawaii \\
TempLAMA & Dhingra et al. & 2012 Cristiano Ronaldo plays for \textit{MASK} where \textit{[MASK]} = Real Madrid \\
& & 2019 Cristiano Ronaldo plays for \textit{MASK} where \textit{[MASK]} = Juventus FC \\
BIOLAMA & Sung et al. & Amantadine has effects on \textit{[MASK]} where \textit{[MASK]} = Parkinson's disease, ... \\





\bottomrule
\end{tabular}}
\end{table*}

==> Survey_ LMs as KB/tables/reasoning_table.tex <==
% \begin{table*}[t]
% \begin{tabular}{lll}
% \toprule
% Reasoning Type & Example                                                 & Answer                      \\
% \midrule
% Logical        & Alice is quiet. Bob is loud. Q: Are Alice and Bob loud? & Alice and Bob are not loud. \\
% Mathematical   & Solve -42*r + 27*c = -1167 and 130*r + 4*c = 372 for r. & 4                           \\
% Commonsense    & Birds can {[}MASK{]}.                                   & fly                        
% \end{tabular}
% \caption{Types of reasoning that KBs are able to do.}
% \end{table*}

% \begin{table*}[]
% \begin{tabular}{|lll|}
% \hline
% \textbf{Reasoning Type} & \textbf{Example}                                        & \textbf{Answer}             \\ \hline
% Logical                 & Alice is quiet. Bob is loud. Q: Are Alice and Bob loud? & Alice and Bob are not loud. \\ \hline
% Mathematical            & Solve -42*r + 27*c = -1167 and 130*r + 4*c = 372 for r. & 4                           \\ \hline
% Commonsense             & Birds can {[}MASK{]}.                                   & fly                         \\ \hline
% \end{tabular}
% \caption{Types of reasoning that KBs are able to do.}

% \end{table*}

\begin{table*}[]
\centering
\begin{tabular}{lll}
\toprule
\textbf{Reasoning Type} & \textbf{Example}                                        & \textbf{Answer}             \\ \midrule
Logical                 & Alice is quiet. Bob is loud. Q: Are Alice and Bob loud? & 
No \\ \hline
Mathematical            & Solve -42*r + 27*c = -1167 and 130*r + 4*c = 372 for r. & 4                           \\ \hline
Commonsense             & Birds can {[}MASK{]}.                                   & fly                         \\ \hline
\end{tabular}
\caption{Types of reasoning that KBs are able to do.}

\end{table*}

==> Survey_ LMs as KB/tables/tasks_to_datasets.tex <==
\begin{table*}[t]
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
& \textbf{Open-Domain QA} & \textbf{Entity Linking} & \textbf{Relation Extraction} & \textbf{Fact Verification} & \textbf{Dialog Generation} & \textbf{Knowledge Embedding} \\ 
\midrule
\textbf{T-REx} & & & \checkmark & & & \\
\textbf{zsRE} & & & \checkmark & & & \\
\textbf{Natural Questions} & \checkmark & & & & & \\
\textbf{FEVER} & & & & & \checkmark & & \\
\textbf{CLIMATE-FEVER} & & & & \checkmark & & \\
\textbf{FEVEROUS} & & & & & & \\
\textbf{Wikidata5m} & & & & & & \checkmark\\
\textbf{TabFact} & & & & \checkmark & & \\
\textbf{ParaRel} & & & & \checkmark & & \\
\textbf{FRUIT-WIKI} & & & & \checkmark & & \\
\textbf{TriviaQA} & \checkmark & & & & & \\

\midrule
\textbf{KILT} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \\



\bottomrule
\end{tabular}}
\end{table*}

==> tables/probes.tex <==
\begin{table*}[t]
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcc}
\toprule
\textbf{Task Name} & \textbf{Paper} & \textbf{Examples} \\ 
\midrule
LAMA & Petroni et al. & Obama was born in \textit{[MASK]}, where \textit{[MASK]} = Hawaii \\
TempLAMA & Dhingra et al. & 2012 Cristiano Ronaldo plays for \textit{MASK} where \textit{[MASK]} = Real Madrid \\
& & 2019 Cristiano Ronaldo plays for \textit{MASK} where \textit{[MASK]} = Juventus FC \\
BIOLAMA & Sung et al. & Amantadine has effects on \textit{[MASK]} where \textit{[MASK]} = Parkinson's disease, ... \\





\bottomrule
\end{tabular}}
\end{table*}

==> tables/reasoning_table.tex <==
% \begin{table*}[t]
% \begin{tabular}{lll}
% \toprule
% Reasoning Type & Example                                                 & Answer                      \\
% \midrule
% Logical        & Alice is quiet. Bob is loud. Q: Are Alice and Bob loud? & Alice and Bob are not loud. \\
% Mathematical   & Solve -42*r + 27*c = -1167 and 130*r + 4*c = 372 for r. & 4                           \\
% Commonsense    & Birds can {[}MASK{]}.                                   & fly                        
% \end{tabular}
% \caption{Types of reasoning that KBs are able to do.}
% \end{table*}

% \begin{table*}[]
% \begin{tabular}{|lll|}
% \hline
% \textbf{Reasoning Type} & \textbf{Example}                                        & \textbf{Answer}             \\ \hline
% Logical                 & Alice is quiet. Bob is loud. Q: Are Alice and Bob loud? & Alice and Bob are not loud. \\ \hline
% Mathematical            & Solve -42*r + 27*c = -1167 and 130*r + 4*c = 372 for r. & 4                           \\ \hline
% Commonsense             & Birds can {[}MASK{]}.                                   & fly                         \\ \hline
% \end{tabular}
% \caption{Types of reasoning that KBs are able to do.}

% \end{table*}

\begin{table*}[]
\centering
\begin{tabular}{lll}
\toprule
\textbf{Reasoning Type} & \textbf{Example}                                        & \textbf{Answer}             \\ \midrule
Logical                 & Alice is quiet. Bob is loud. Q: Are Alice and Bob loud? & 
No \\ \hline
Mathematical            & Solve -42*r + 27*c = -1167 and 130*r + 4*c = 372 for r. & 4                           \\ \hline
Commonsense             & Birds can {[}MASK{]}.                                   & fly                         \\ \hline
\end{tabular}
\caption{Types of reasoning that KBs are able to do.}

\end{table*}

==> tables/tasks_to_datasets.tex <==
\begin{table*}[t]
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
& \textbf{Open-Domain QA} & \textbf{Entity Linking} & \textbf{Relation Extraction} & \textbf{Fact Verification} & \textbf{Dialog Generation} & \textbf{Knowledge Embedding} \\ 
\midrule
\textbf{T-REx} & & & \checkmark & & & \\
\textbf{zsRE} & & & \checkmark & & & \\
\textbf{Natural Questions} & \checkmark & & & & & \\
\textbf{FEVER} & & & & & \checkmark & & \\
\textbf{CLIMATE-FEVER} & & & & \checkmark & & \\
\textbf{FEVEROUS} & & & & & & \\
\textbf{Wikidata5m} & & & & & & \checkmark\\
\textbf{TabFact} & & & & \checkmark & & \\
\textbf{ParaRel} & & & & \checkmark & & \\
\textbf{FRUIT-WIKI} & & & & \checkmark & & \\
\textbf{TriviaQA} & \checkmark & & & & & \\

\midrule
\textbf{KILT} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \\



\bottomrule
\end{tabular}}
\end{table*}
